Towards Tight Bounds for Spectral Sparsification of Hypergraphs

Cut and spectral sparsification of graphs have numerous applications, including e.g. speeding up algorithms for cuts and Laplacian solvers. These powerful notions have recently been extended to hypergraphs, which are much richer and may offer new applications. However, the current bounds on the size of hypergraph sparsifiers are not as tight as the corresponding bounds for graphs. Our first result is a polynomial-time algorithm that, given a hypergraph on $n$ vertices with maximum hyperedge size $r$, outputs an $\epsilon$-spectral sparsifier with $O^*(nr)$ hyperedges, where $O^*$ suppresses $(\epsilon^{-1} \log n)^{O(1)}$ factors. This size bound improves the two previous bounds: $O^*(n^3)$ [Soma and Yoshida, SODA'19] and $O^*(nr^3)$ [Bansal, Svensson and Trevisan, FOCS'19]. Our main technical tool is a new method for proving concentration of the nonlinear analogue of the quadratic form of the Laplacians for hypergraph expanders. We complement this with lower bounds on the bit complexity of any compression scheme that $(1+\epsilon)$-approximates all the cuts in a given hypergraph, and hence also on the bit complexity of every $\epsilon$-cut/spectral sparsifier. These lower bounds are based on Ruzsa-Szemer\'edi graphs, and a particular instantiation yields an $\Omega(nr)$ lower bound on the bit complexity even for fixed constant $\epsilon$. This is tight up to polylogarithmic factors in $n$, due to recent hypergraph cut sparsifiers of [Chen, Khanna and Nagda, FOCS'20]. Finally, for directed hypergraphs, we present an algorithm that computes an $\epsilon$-spectral sparsifier with $O^*(n^2r^3)$ hyperarcs, where $r$ is the maximum size of a hyperarc. For small $r$, this improves over $O^*(n^3)$ known from [Soma and Yoshida, SODA'19], and is getting close to the trivial lower bound of $\Omega(n^2)$ hyperarcs.

==> 360-general-sparsification.tex <==
%!TEX root=./000-main.tex

\subsection{General sparsification}
\label{sec:general-sparsification}


\begin{lemma}\label{lem:partition}
Let $G=(V,E)$ be an $r$-uniform hypergraph with $n$ vertices and $m$ edges. Then there exists a partion of $V$ into disjoint vertex sets $C_1,\ldots, C_k$ that satisfies the following:

Let $E_j$ be the multiset of edges supported on $C_j$ and let $G_j=(C_j,E_j)$ and let $E_0=E\setminus\bigcup_{j=1}^k E_j$. Then
\begin{enumerate}
    \item for all $j$, $\Phi(G_j) = \Omega(1/(r\log^2 n))$,
    \item $|E_0|\le m/2$,
    \item for all $j$, $\min_{v\in C_j}d_{G_j}(v)\ge m/4n$.
\end{enumerate}

Let $\textsc{ExpanderDecompsition}(G)$ return such a collection.
\end{lemma}
We defer the proof of Lemma~\ref{lem:partition} to Section~\ref{subsec:expander-decomposition}.

\begin{lemma}\label{lem:expander-sparsify}
Let $G=(V,E)$ be an $r$-uniform hypergraph with expansion $\Phi(G)\ge\tfrac1{r\log	^2n}$. Then there exists an $\epsilon$-spectral sparsifier of $G$ with at most $(n-1)r(\epsilon^{-1}\log n)^{O(1)}$ edges.

Let $\textsc{ExpanderSparsify}(G,\epsilon)$ return such a sparsifier.
\end{lemma}

\begin{proof}
	This is a simple corollary of Theorem~\ref{thm:expander-sparsification} when applied with $\Phi=\tfrac1{r\log^2n}$. The only difference is the $(n-1)$ instead of the $n$ in the formula. This difference is only meaningful in the edge case when $n=1$, where enforce the sparsifier to be empty (this is indeed a spectral sparsifier of any graph on one vertex). The reason for dealing with this edge case separately will become clear in the proof of Theorem~\ref{thm:general-sparsification} below.
\end{proof}

\begin{definition}\label{def:tr-cl}
Let $\sim$ be a relation on a ground set $V$. The transitive closure $\approx$ of $\sim$ is a relation on $U$ defined as follows
$$a\approx b\ \Longleftrightarrow\ \exists c_1,\ldots,c_k\in V, a\sim c_1\sim\cdots\sim c_k\sim b.$$
\end{definition}

\begin{definition}\label{def:contract}
Let $G=(V,E)$ be a hypergraph and let $\approx$ be an equivalence relation on $V$.
Then contraction of $G$ with respect to $\approx$, denoted $G/\approx$, is a graph on the vertex set $V'=V/\approx$ and the edge multiset
$$E'=\{\{[v] \mid v\in e\} \mid e\in E\},$$
where $[v]$ denotes the equivalence class of $v$ with respect to $\approx$. That is, for example if $e$ contained both $u$ and $v$ in the original graph, where $u\approx v$, then in the contraction $e$ contains $[u]=[v]$ with multiplicity at least $2$. In what follows, we will often slightly abuse notation and equate the edges of $E$ and $E'$.
\end{definition}

\begin{observation}\label{obs:contraction-sparsification}
	Let $G=(V,E)$ be a hypergraph and let $\approx$ be an equivalence relation on $V$. Let $\widetilde G$ be an $\epsilon$-spectral sparsifier not of $G$, but of $G/\approx$. Then the energy of $G$ is not necessarily well approximated by the energy of $\widetilde G$ on all $x\in\mathbb R^V$, in the sense that
	$$\widetilde Q(x)=(1\pm\epsilon)Q(x).$$
	However, the above equation does hold if $x$ is constant on all equivalence classes of $\approx$, that is if
	$$u\approx v\ \Rightarrow\ x_u=x_v.$$
\end{observation}

\begin{algorithm}[H]
\label{alg:main}
\caption{Algorithm sparsifying arbitrary hypergraph}
\begin{algorithmic}[1]
\Procedure{Sparsify}{$G,\epsilon$}
    \State $E^{(0)}\gets E$.
    \State $\widetilde E\gets\emptyset$.
    \State $i\gets0$.
    \For{$i=0,\ldots,\log m$}
        \If{$i>5\log n$}
            \State Define a relation $\sim_i$ so that $u\sim_i v$ iff $\exists i'\le i-5\log n,\ \exists j, \ [u],[v]\in C^{(i')}_j$.\label{line:sim-def}
            \State $\approx_i\gets\text{transitive closure of}\sim_i$.
            \State $G^{(i)}\gets(V,E^{(i)})/\approx_i$.
        \Else
            \State $G^{(i)}\gets(V,E^{(i)})$.
        \EndIf
        \State $\left(C^{(i)}_1\ldots,C^{(i)}_{k_i}\right)\gets\textsc{ExpanderDecomposition}(G^{(i)})$.
        \For{$j=1\ldots k_i$}
            \State $E_j^{(i)}\gets$ the subset of $E^{(i)}$ that is supported on $C_j^{(i)}$. 
            \State $G_j^{(i)}=(C_j^{(i)},E_j^{(i)})$.
            \State $(C_j^{(i)},\widetilde E_j^{(i)})=\textsc{ExpanderSparsify}(G_j^{(i)},\epsilon/10)$.\label{line:def-tilde-Eij}
            \State $\widetilde E\gets \widetilde E\cup \widetilde E_j^{(i)}$.\label{line:update-tilde-E}
        \EndFor
        \State $E^{(i+1)}\gets E^{(i)}\setminus\cup_{j=1}^{k_i}E_j^{(i)}$.\label{line:remove-edges}
    \EndFor
    \State \Return $\widetilde G=(V,\widetilde E)$.
\EndProcedure
\end{algorithmic}
\end{algorithm}

In line~\ref{line:sim-def}, $[u],[v]\in C_j^{(i')}$ means that the \textit{supernodes containing $u$ and $v$} where in the same expander of the decomposition at level $i'$. Note also the abuse of notation in lines~\ref{line:def-tilde-Eij} and~\ref{line:update-tilde-E}: In line~\ref{line:def-tilde-Eij}, $\widetilde E_j^{(i)}$ is defined as a multiset of edge on the \textit{contracted} vertex set $C_j^{(i)}\subseteq V/\approx_i$, but on line~\ref{line:update-tilde-E}, we treat it containing edges supported on $V$. Since elements of $\widetilde E_j^{(i)}$ have clearly corresponding counterparts in $E$, we don't further complicate notation by making this distinction formal.

Also note that throughout the contractions, our graphs always remain $r$-regular, thanks to the use of multisets as edges (see Definition~\ref{def:contract}). This allows use \textsc{ExpanderSparsify} in line~\ref{line:def-tilde-Eij}.


\begin{theorem}\label{thm:general-sparsification}
Let $G=(V,E)$ be an $r$-uniform hypergraph. Then $\textsc{Sparsify}(G,\epsilon)$ returns an $\epsilon$-spectral sparsifier of $G$ with $O(nr(\epsilon^{-1}\log n)^{O(1)})$ edges.
\end{theorem}

First let us consider the size of the saprsifier output by $\textsc{Sparsify}(G,\epsilon)$.
In the hypergraph $\widetilde G=(V,\widetilde E)$, $\widetilde E$ is simply the union of $\widetilde E_j^{(i)}$ for all $i$ and $j$, and by Lemma~\ref{lem:expander-sparsify} the size of $\widetilde E_j^{(i)}$ is at most $|C_j^{(i)}-1|r(\epsilon\log|C_j^{(i)})^{O(1)}|\le|C_j^{(i)}-1|r(\epsilon\log n)^{O(1)}$. To bound the size of $\widetilde G$ we need to bound
$$\sum_{i=0}^{\log m}\sum_{j=1}^{k_i}|C_j^{(i)}-1|.$$

\begin{claim}
$$\sum_{i=0}^{\log m}\sum_{j=1}^{k_i}|C_j^{(i)}-1|\le10n\log n$$
\end{claim}
\begin{proof}
To do this, we will first bound the number of vertices (including supernodes) that exist throughout Algorithm~\ref{alg:main},
$$V^*=\bigcup_{i=0}^{\log m}\bigcup_{j=1}^{k_i}C_j^{(i)}.$$
This set includes all the vertices from $V$, as well as some contracted supernodes, that are subsets of $V$. Note however, that these sets form a laminar family, since supernodes are only constructed by merging previous supernodes - no supenodes ever get broken apart. Therefore, $|V^*|\le2n-1$.

It now suffices to bound the number of \textit{non-singleton} clusters a single $v\in V^*$ can participate in. As soon as $v$ participates in some cluster $C$ of size at least $2$ at level $i$, we know that at level $i+5\log n$ $C$ will be contracted into a different vertex in $V^*$. Therefore, $v$ can participate in at most $5\log n$ clusters of size $2$ or more. Therefore, the total of the sum is at most
$$(2n-1)\cdot5\log n\le10\log n.$$
\end{proof}

As a corollary, we get that the number of hyperedges in $\widetilde E$ is indeed at most $nr(\epsilon^{-1}\log n)^{O(1)}$.

We turn now to proving the quality of $\widetilde G$ is a spectral sparsifier. Using the additiviy of spectral sparsifiers, it safices to prove separately that for each $i$ and $j$, $(V,\widetilde E_j^{(i)})$ is an $\epsilon$-spectral sparsifier to $(V,E_j^{(i)})$. We must first verify that each hyperedge of $E$ appears in exactly one of $E_j^{(i)}$. Indeed, any hyperedge can appear in at most one of them: $E_j^{(i)}$ gets removed from $E^{(i+1)}$ at the end of the main for loop in line~\ref{line:remove-edges}. Furthermore, all hyperedges eventually get removed this way: By Lemma~\ref{lem:partition}, after each round no more than half the edges remain, so after $\log m+1$ rounds all hyperedges must be gone and $E^{(\log m+1)}=\emptyset$.

Let us focus on a single cluster $C_j^{(i)}$ and compare the spectral properties of $E_j^{(i)}$ and $\widetilde E_j^{(i)}$. At this point it is important to keep in mind the difference between the graphs $\widehat G_j^{(i)}=\left(V,E_j^{(i)}\right)$, $G_j^{(i)}=\left(C_j^{(i)},E_j^{(i)}\right)$, $\widetilde G_j^{(i)}=\left(C_j^{(i)},\widetilde E_j^{(i)}\right)$, and $\breve G_j^{(i)}=\left(V,\widetilde E_j^{(i)}\right)$. Though $\widehat G_j^{(i)}$ and $G_j^{(i)}$ share their edge multiset, they are not the same, in fact $G_j^{(i)}=\widehat G_j^{(i)}/\approx_i$. Similarly, $\widetilde G_j^{(i)}=\breve G_j^{(i)}/\approx_i$. Lemma~\ref{lem:expander-sparsify} says that $\widetilde G_j^{(i)}$ is an $\epsilon$-spectral sparsifier to $G_j^{(i)}$, it makes no such guarantee about $\widehat G_j^{(i)}$ and $\breve G_j^{(i)}$.

We must show that for any vector $x\in\mathbb R^V$ we have
\begin{equation}\label{eq:general-main}
\breve Q(x)=(1\pm\epsilon)\cdot \widehat Q(x),
\end{equation}
where $\widehat Q$ and $\breve Q$ denote the energy with respect to $\widehat G_j^{(i)}$ and $\breve G_j^{(i)}$ respectively. Recall from Observation~\ref{obs:contraction-sparsification} that equation~\ref{eq:general-main} holds when $x$ is constant within all supernodes of $C_j^{(i)}$. Our plan is therefore to round round $x$ to $\widetilde x$ such that it satisfies this requirement and then show informally that
$$\widehat Q(x)\approx\widehat Q(\widetilde x)\approx\breve Q(\widetilde x)\approx\breve Q(x).$$

We may assume that without loss of generality that $i>\log n$, as otherwise no contraction takes place and equation~\ref{eq:general-main} simply holds. Let $\delta$ be the maximum discrepancy between the values of $x$ within supernodes of $C_j^{(i)}$, that is
$$\delta=\max_{u\approx_i|x_u-x_v|}|x_u-x_v|.$$
Our rounding of $x$ to $\widetilde x$ is mostly arbitrary, we enforce only that no coordinate changes by more than an additive $\delta$.

\begin{claim}
For any edge $e$ in $E_j^{(i)}$
	$$\widehat Q_{\widetilde x}(e)=(1\pm\epsilon/10)\widehat Q_x(e)\pm\frac{\epsilon Q(x)}{10m_in},$$
	where $m_i$ is the size of $E^{(i)}$ and $Q(x)$ is the quadratic form for the entire input graph $G$.
\end{claim}

\begin{proof}
	
	Recall that the the additive error between $x$ and $\widetilde x$ is at most $\delta$, so by Lemma~\ref{lem:additive-error}
	$$\big|\widehat Q_x(e)-\widehat Q_{\widetilde x}(e)\big|
	\le 4\delta\left(\sqrt{\widehat Q_x(e)}+\delta\right).$$
	
	We distinguish between two cases based on the size of $\sqrt{\widehat Q_x(e)}$ relative to $\delta$. First suppose that $\delta\le\epsilon\sqrt{\widehat Q_x(e)}/50$. This is the simpler case, as we can just substitute this upper bound in for delta in the formula above:
	$$\big|\widehat Q_x(e)-\widehat Q_{\widetilde x}(e)\big|
	\le4\epsilon\sqrt{\widehat Q_x(e)}/50\cdot\left(\sqrt{\widehat Q_x(e)}+\epsilon\sqrt{\widehat Q_x(e)}/50\right)
	\le\epsilon\widehat Q_x(e)/10,$$
	as claimed.
	
	Now suppose $\delta\ge\epsilon\sqrt{\widehat Q_x(e)}/50$. This time, we substitute in for $\widehat Q_x(e)$ to get
	$$\big|\widehat Q_x(e)-\widehat Q_{\widetilde x}(e)\big|
	\le4\delta\left(50\delta/\epsilon + \delta\right)
	\le204\delta^2/\epsilon.$$
	
	



Based on the definition of $\delta$, let $u,v\in V$ be such that $u\approx_i v$ and $|x_u-x_v|=\delta$.
By Definition~\ref{def:tr-cl} there must exist a path of vertices $u,w_1,\ldots,w_k,v$ such that $u \sim_i w_1$, $w_k\sim_i v$, and $w_\ell\sim_i w_{\ell+1}$ for all $\ell \in [k-1]$ ($\sim_i$ is defined in Line~\ref{line:sim-def}).
Choose $\ell$ such that $|x_{w_\ell}-x_{w_{\ell+1}}|\ge\delta/n$ (since the length of the path is at most $n$). By definition of $\sim_i$, there exists $i'\le i -5\log n$ and $j'$ such that $w_{\ell},w_{\ell+1}\in C_{j'}^{(i')}$, but $w_\ell\not\sim_{i'}w_{\ell+1}$.

We can lower bound $Q(x)$ be the energy of $x$ with respect to $G_{j'}^{(i')}$ specifically. To lower bound the energy of $x$ on $G_{j'}^{(i')}$, we can apply hypergraph Cheeger (Theorem~\ref{thm:hypergraph-cheeger}). We know by the first guarantee of \textsc{ExpanderDecomposition} that $\Phi\left(G_j^{(i')}\right)\ge\tfrac{1}{r\log^2n}$. Let the number of edges remaining $E^{(i')}$ be $m_{i'}$. Therefore, by the third guarantee of \textsc{ExpanderDecomposition}, the minimum degree of $G_{j'}^{i'}$ is at least $m_{i'}/4n$. In general, the hypergraph Cheeger inequality states that when $x$ in centered (that is $\sum_{v\in V}x_v=0$)
$$Q(x)\ge\frac{r\Phi^2}{32}\sum dx^2.$$
Our vector $x$ is not centered with respect to the cluster $C_{j'}^{(i')}$. However, since the difference between $x_{w\ell}$ and $x_{w_{\ell+1}}$ is $\delta$, at least one of them will have absolute value at least $\delta/2$ even when $x$ \textit{is} centered. Therefore,
$$Q_{C_{j'}^{(i')}}(x)\ge \frac{r\cdot\left(\tfrac1{r\log^2n}\right)^2}{32}\cdot\frac{m_{i'}}{4n}\cdot(\delta/2)^2,$$
just by looking at the terms corresponding to $w_\ell$ and $w_{\ell+1}$.

Thus we have
\begin{align*}
\big|\widehat Q_x(e)-\widehat Q_{\widetilde x}(e)\big|&\le204\delta^2/\epsilon\\
&\le204/\epsilon\cdot4\cdot\frac{32}{r\cdot\left(\tfrac1{r\log^2n}\right)^2}\cdot\frac{4n}{m_{i'}}\cdot Q(x)\\
&\le\frac{110000nr\log^2n}{\epsilon m_{i'}}\cdot Q(x)
\end{align*}

To relate this to $m_i$, as stated in the claim, recall that by the second property of \textsc{ExpanderDecomposition} the total number of hyperedges decreases at least by a factor of $2$ during every iteration of the outer for-loop. So, since $i'\le i-50\log n$, we have that $m_i\le m_in^{-5}$, and
$$\big|\widehat Q_x(e)-\widehat Q_{\widetilde x}(e)\big|\le\frac{10000nr\log^2n}{\epsilon m_in^5}\le\frac{\epsilon Q(x)}{m_in},$$
since $1100000\log^2n$, $r$ and $\epsilon^{-1}$ are all smaller than $n$, by the theorem hypothesis, and for large enough $n$.

Putting the two cases together gives us the additive and multiplicative errors terms and proves the claim.


\end{proof}



\begin{claim}\label{claim:g1}
	$$\widehat Q(\widetilde x)=\left(1\pm\frac{\epsilon}{10}\right)\widehat Q(x)\pm\frac{\epsilon Q(x)}{10n}$$
\end{claim}

\begin{proof}
	\jnote{TODO}
\end{proof}

\begin{claim}\label{claim:g2}
$$\breve Q(\widetilde x)=\left(1\pm\frac{\epsilon}{10}\right)\widehat Q(\widetilde x)$$
\end{claim}
\begin{proof}
As mentioned above equation~\ref{eq:general-main} holds when $x$ (in this case $\widetilde x$) is constant on all equivalence classes of $\approx_i$.
\end{proof}

\begin{claim}\label{claim:g3}
$$\breve Q(\widetilde x)=\left(1\pm\frac{\epsilon}{10}\right)\breve Q(x)\pm\frac{2\epsilon Q(x)}{10n}$$
\end{claim}
\begin{proof}
	\jnote{TODO}
\end{proof}

By combining Claims~\ref{claim:g1},~\ref{claim:g2}, and~\ref{claim:g3} we get the statement of the lemma.


